Phoenix: A Formally Verified Regenerating Vault

An attacker that gains access to a cryptocurrency user's private keys can perform any operation in her stead. Due to the decentralized nature of most cryptocurrencies, no entity can revert those operations. This is a central challenge for decentralized systems, illustrated by numerous high-profile heists. Vault contracts reduce this risk by introducing artificial delay on operations, allowing abortion by the contract owner during the delay. However, the theft of a key still renders the vault unusable and puts funds at risk. We introduce Phoenix, a novel contract architecture that allows the user to restore its security properties after key loss. Phoenix takes advantage of users' ability to store keys in easily-available but less secure storage (tier-two) as well as more secure storage that is harder to access (tier-one). Unlike previous solutions, the user can restore Phoenix security after the theft of tier-two keys and does not lose funds despite losing keys in either tier. Phoenix also introduces a mechanism to reduce the damage an attacker can cause in case of a tier-one compromise. We formally specify Phoenix's required behavior and provide a prototype implementation of Phoenix as an Ethereum contract. Since such an implementation is highly sensitive and vulnerable to subtle bugs, we apply a formal verification tool to prove specific code properties and identify faults. We highlight a bug identified by the tool that could be exploited by an attacker to compromise Phoenix. After fixing the bug, the tool proved the low-level executable code's correctness.

==> ledger_figure.tex <==
% I couldn't center this figure, so I added it as an image. Code is here in case we want to alter this figure later.

\begin{figure}[!h]
\tikzstyle{block} = [rectangle, draw, text width=5em, text centered, rounded corners, minimum height=4em, fill=gray!30, minimum width=2.5cm, align=center]
\tikzstyle{line} = [draw, -latex]
\begin{tikzpicture}[node distance=1cm, auto]

    \node (init) {};
    
    % Top of chart - map block with entering ID arrow
    \node [block] (map) {Map\\ \includegraphics[width=.35\textwidth]{dictionary.png}};
    \coordinate [left=2.5cm of map] (UL);
    \path [line]   (UL) -- node [text width=2.5cm,midway,above,align=center ] {query ID} (map);
    
    % head block
    \node [block] (head) [below left=1.7cm and 1.45cm of map] {\scriptsize \textbf{\textit{Request}}\\
    ID\\
    amount\\
    recipient\\
    creation\_block\\
    initiator
    \par};
    \coordinate [left=1cm of head] (LL);
    \path [line]   (LL) -- node [text width=2.5cm,midway,above,align=center ] {head} (head);
    
    % query block #2
    \node [block] (node2) [right=1.4cm of head.east] {\scriptsize \textbf{\textit{Request}}\\
    ID\\
    amount\\
    recipient\\
    creation\_block\\
    initiator
    \par};
    
    % Arrows between head and query block #2
    \path [line] ([shift={(0,4mm)}]head.east) -- node [text width=1.4cm, midway, above, align=center ] {previous} ([shift={(0,4mm)}]node2.west);
    \path [line] ([shift={(0,-4mm)}]node2.west) -- node [text width=1.4cm, midway, above, align=center ] {next} ([shift={(0,-4mm)}]head.east);
    
    % etc. node
    \node [block] (etc) [right=1.4cm of node2.east] {...};
    
    % Arrows between node #2 and etc. node
    \path [line] ([shift={(0,4mm)}]node2.east) -- node [text width=1.4cm, midway, above, align=center ] {previous} ([shift={(0,4mm)}]etc.west);
    \path [line] ([shift={(0,-4mm)}]etc.west) -- node [text width=1.4cm, midway, above, align=center ] {next} ([shift={(0,-4mm)}]node2.east);
    
    % Marking linked list
    \node [dashed, draw=black, rounded corners, fill=none, align=center, label=below:{Linked list}, fit=(head) (etc)] {};
    
    % Pointers to list from map
    \path [line]   (map) -- node [text width=1cm, midway, above, align=center, fill=white ] {ptr*} (head);

    \path [line]   (map) -- node [text width=1cm, midway, above, align=center, fill=white ] {ptr*} (node2);
    
    \path [line]   (map) -- node [text width=1cm, midway, above, align=center, fill=white ] {ptr*} (etc);
\end{tikzpicture}

\caption{Ledger structure} \label{fig:Ledger}
\end{figure}
